Robust Distortion-free Watermarks for Language Models

We propose a methodology for planting watermarks in text from an autoregressive language model that are robust to perturbations without changing the distribution over text up to a certain maximum generation budget. We generate watermarked text by mapping a sequence of random numbers -- which we compute using a randomized watermark key -- to a sample from the language model. To detect watermarked text, any party who knows the key can align the text to the random number sequence. We instantiate our watermark methodology with two sampling schemes: inverse transform sampling and exponential minimum sampling. We apply these watermarks to three language models -- OPT-1.3B, LLaMA-7B and Alpaca-7B -- to experimentally validate their statistical power and robustness to various paraphrasing attacks. Notably, for both the OPT-1.3B and LLaMA-7B models, we find we can reliably detect watermarked text ($p \leq 0.01$) from $35$ tokens even after corrupting between $40$-$50\%$ of the tokens via random edits (i.e., substitutions, insertions or deletions). For the Alpaca-7B model, we conduct a case study on the feasibility of watermarking responses to typical user instructions. Due to the lower entropy of the responses, detection is more difficult: around $25\%$ of the responses -- whose median length is around $100$ tokens -- are detectable with $p \leq 0.01$, and the watermark is also less robust to certain automated paraphrasing attacks we implement.

==> preamble.tex <==
\usepackage[utf8]{inputenc} % allow utf-8 input
\usepackage{geometry}
\geometry{verbose,tmargin=1in,bmargin=1in,lmargin=3cm,rmargin=3cm}
\usepackage{float}

\usepackage[english]{babel}
\usepackage{array}
\usepackage{verbatim}
\usepackage{diagbox}
\usepackage{enumitem}
\usepackage{xifthen}

\usepackage{amsmath, amsfonts, amsthm, bm,  amssymb, longtable, multirow, mathrsfs}
% \usepackage{epstopdf, graphicx, subcaption, dsfont}
% \usepackage{algorithm}  
% \usepackage{algorithmicx}  
\usepackage{algpseudocode}
\usepackage{booktabs}
\usepackage{array}
\usepackage{booktabs}
\usepackage[numbers]{natbib}

\usepackage{setspace}
%% \onehalfspacing
% \usepackage{parskip}

\usepackage{xcolor}

\usepackage[ruled,linesnumbered,noend]{algorithm2e}

% \usepackage{cleveref}

\definecolor{darkblue}{rgb}{0,0,.5}
\RequirePackage[colorlinks,allcolors=darkblue]{hyperref}

\usepackage[capitalize]{cleveref}
\usepackage{crossreftools}

\allowdisplaybreaks

\theoremstyle{plain}
\newtheorem{theorem}{Theorem}

\newtheorem{lemma}{Lemma}[section]
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{corollary}{Corollary}
\newtheorem{observation}{Observation}[section]
\newtheorem{claim}[lemma]{Claim}

\theoremstyle{definition}

\newtheorem{assumption}{Assumption}
\renewcommand{\theassumption}{A\arabic{assumption}}
\newtheorem{definition}{Definition}

\theoremstyle{remark}
\newtheorem*{rem}{Remark}
\newtheorem*{note}{Note}

\newcounter{example}
\newenvironment{example}[1][]{
  \refstepcounter{example}
  \ifthenelse{\isempty{#1}}{%
    % There is no text to display in the example
    \noindent \textbf{Example \theexample:}\hspace*{.05em}
  }{%
    \noindent \textbf{Example \theexample} ({#1})\textbf{:}\hspace*{.05em}
  }
}{%
  $\Diamond$ \medskip
}


\newenvironment{sproof}{\renewcommand{\proofname}{Proof sketch}\proof}{\endproof}

\newcommand{\tabincell}[2]{\begin{tabular}{@{}#1@{}}#2\end{tabular}}

\let\oldnl\nl% Store \nl in \oldnl
\newcommand{\nonl}{\renewcommand{\nl}{\let\nl\oldnl}}% Remove line number for one line

\newlength{\phaserulewidth}
\newcommand{\setphaserulewidth}{\setlength{\phaserulewidth}}
\newcommand{\phase}[1]{
  %
  % Top phase rule
  \nonl\hrulefill\\
  \nonl\strut#1\\% Phase text
  % Bottom phase rule
  % \nonl\vspace{-1.25ex}\leavevmode\rule{\linewidth}{\phaserulewidth}\;
  \nonl\vspace{-1.25ex}\hrulefill\\
}
\setphaserulewidth{.7pt}

\usepackage{listings}
\usepackage{amssymb}

==> sections/app-stealth.tex <==
\section{Proof of Lemma~\ref{thm:stealth}}\label{app:stealth}
\rck{ignore the appendix for now}


==> sections/prelims.tex <==
% \section{Preliminaries}
% \subsection{Notation}
% Let $\mc{V} = [n]$ be the \textit{vocabulary},
% where $n \in \N$ is the size of the vocabulary (i.e., number of tokens).
% Let $f : \(\emptyset \cup \mc{V}^*\) \to \Delta(\mc{V}) =: \mc{F}$
% denote an (autoregressive) \textit{language model} 
% that takes a prefix of arbitrary length as input and returns a 
% distribution over the vocabulary, i.e., an element of the $n$-dimensional 
% probabability simplex, and for $m \in N$ let $P_f^m(\cdot \mid p)$ denote the 
% distribution over sequences of length $m$ induced by 
% sampling autoregressively from the language model $f$ conditional 
% on the prefix $p$.

% \subsection{Problem formulation}
% Given an arbitrary language model $f$, our goal is to give a
% collection of watermarked language models $f_\xi := \(\emptyset \cup \mc{V}^*\)
% \to \Delta(\mc{V})$ indexed by $\xi \in \Xi$ along with a distribution $P_\xi$ over $\Xi$ 
% such that $\xi \sim P_\xi$ and $S \sim \P_{f_\xi}^m(\cdot \mid p)$
% satisfy the following conditions for any prefix 
% $p \in \(\emptyset \cup \mc{V}^*\)$ and sufficiently large sequence length $m$:
% \begin{itemize}
%     \item[(C.i)] $S \stackrel{d}{=} S'$ for $S' \sim P_f^m(\cdot \mid p)$,
%     \item[(C.ii)] $D_{TV}((S,\xi)||(S',\xi)) \geq 1-\delta$
%                     for $S' \sim P_f^m(\cdot \mid p)$.
% \end{itemize}

% Thinking of $\xi$ as a source of additional randomness, the
% (marginal) distribution over sequences induced by the collection of watermarked language models 
% should be the same as the distribution induced by the original language model,
% but anyone who observes $\xi$ should be able to easily distinguish between the watermarked 
% versus unwatermarked text.
% Eventually, we will replace the randomness in $P_\xi$ with pseudorandomness; 
% the idea is that so long 
% as the pseudorandomness is indistinguishable from the original randomness,
% the two conditions will still hold (at least approximately).

